Nooks: Social Spaces to Lower Hesitations in Interacting with New People at Work

Initiating conversations with new people at work is often intimidating because of uncertainty about their interests. People worry others may reject their attempts to initiate conversation or that others may not enjoy the conversation. We introduce a new system, Nooks, built on Slack, that reduces fear of social evaluation by enabling individuals to initiate any conversation as a nook -- a conversation room that identifies its topic, but not its creator. Automatically convening others interested in the nook, Nooks further reduces fears of social evaluation by guaranteeing individuals in advance that others they are about to interact with are interested in the conversation. In a multi-month deployment with participants in a summer research program, Nooks provided participants with non-threatening and inclusive interaction opportunities, and ambient awareness, leading to new interactions online and offline. Our results demonstrate how intentionally designed social spaces can reduce fears of social evaluation and catalyze new workplace connections.

==> sections-old/01_introduction_diff.tex <==
Whether we are attempting to get acquainted with other residents in our dormitory or other coworkers in our office, in many social groups we are part of across personal and professional contexts, we commonly find ourselves wanting to initiate interactions and develop relationships with ``familiar strangers''~\cite{paulos2004familiar, milgram1977familiar}---described by social psychologist Stanley Milgrim as people we regularly observe but do not interact with. Social relationships within a group can have far-reaching consequences---strong relationships with others in the group can transform a group into a source of social support and enhance well-being by allowing individuals to derive positive meaning from their participation in the group. However, even when there is a mutual desire to interact and develop familiarity, initiating interactions with familiar strangers can be challenging for many~\cite{mitchell2019facilitating, olsson2020technologies, mitchell2019levelling, exley2004small, jarusriboonchai2016design}. The difficulty arises from the fact that ``interactions do not simply begin'': individuals must figure out what to talk about and who goes first~\cite{haugh2021pragmatics, olsson2020technologies}. Initiating conversations with unfamiliar others involves risks because 

==> sections-old/01_introduction_v0.tex <==
Whether we are attempting to get acquainted with other residents in our dormitory or other coworkers in our office, across a range of personal and professional contexts, we commonly find ourselves wanting to initiate interactions and develop relationships with ``familiar strangers''~\cite{paulos2004familiar, milgram1977familiar}---described by social psychologist Stanley Milgrim as people we regularly observe but do not interact with. Even when there is a mutual desire to interact and develop familiarity, initiating interactions with these familiar strangers can be challenging for many~\cite{mitchell2019facilitating, olsson2020technologies, mitchell2019levelling, exley2004small, jarusriboonchai2016design}. The difficulty arises from the fact that ``interactions do not simply begin'': individuals must figure out what to talk about, with unknown others~\cite{haugh2021pragmatics, olsson2020technologies}. 

Researchers, designers, and artists have demonstrated the potential of designed icebreaker experiences to help people initiate interactions and develop relationships with others in their social groups,
% including those with whom they may be unacquainted
~\cite{karahalios2004telemurals, hespanhol2014using, chlup2010breaking, depping2016trust, sileo1998strategies, trotto2013engage}.
Designed icebreaker experiences use online and offline approaches to bring people together and spark conversations by providing the group with a shared focus~\cite{ludvigsen2005designing}. To provide this shared focus, they employ various interaction prompts---discussion prompts~\cite{sileo1998strategies, chlup2010breaking}, installations~\cite{karahalios2004telemurals, snibbe2009social, hespanhol2014using}, gadgets~\cite{paulos2004familiar, mitchell2015sensing}, and even games~\cite{jarusriboonchai2016design, nasir2013cooperative}---and occasionally even sequence prompts to become increasingly intimate. Through this designed scaffolding, they contribute \textit{what} a group can talk about and aim to support progressive development of familiarity, solidarity and closeness. [One sentence about how prompts can icrease likelihood of someone saying something] 

Unfortunately the same designed scaffolding that is intended to support initial interactions, can also limit the effectiveness of icebreaking experiences: interaction prompts and sequences impede formation of closeness if some participants are forced into interactions they don't \textit{want} to have. Icebreaking experiences attempt to eliminate barriers around what to talk about by enforcing predefined interaction prompts and sequences. However, even if participants voluntarily participate in the icebreaking experience as a whole, they may not be fully informed of the specific interactions that are to follow--- icebreaking experiences don't explicitly account for what each participant is willing to talk about, in a given group and at a certain point in time. As a result of this, icebreaking experiences can lead to situations where some participants in an interaction find the interaction uninteresting, irrelevant, or even inappropriate~\cite{miller2021meeting, rogers2002subtle}. Successful evolution of early relationships requires self-disclosures accompanied by reciprocal self-disclosures from others in the interaction~\cite{miller2021meeting, sprecher2013taking, svennevig2014direct}. However, if some participants find the prompt inappropriate or irrelevant, it can prevent them from sharing as well as reciprocating the self-disclosures they receive from others~\cite{miller2021meeting}. Additionally, when participants in an interaction fear that others might be uninterested and may not reciprocate their self-disclosures, they may choose not to participate themselves. By muting individual agency in the process of enforcing scaffolding, designed icebreaker experiences---despite their benefits---can often fail at their goal of relationship building.

We propose that icebreaker experiences can better support early relationship formation in social groups if they are augmented with agency-enhancing mechanisms, where
instead of enforcing interaction prompts and sequences, interactions captured what participants \textit{want to} talk about and participants are provided with the choice to opt in to \textit{specific} interactions they want to participate in. When all participants in an interaction want to participate, risk of non reciprocation is lower. Such a mechanism, intuitively, communicates to everyone in an interaction that the interaction is mutually involving: that everyone in the conversation shares a desire to interact on the topic. This can alleviate fears of non-reciprocity and also foster similarity-based affection, both of which can support relationship building~\cite{svennevig2014direct}. The need for icebreaker experiences that are not over-prescriptive and allow participants to appropriate and avoid interactions has been previously acknowledged~\cite{mitchell2019levelling, rogers2002subtle}. However, manually orchestrating such a mechanism in a group can be cumbersome, requiring effort to source potential interaction prompts, periodically check with each person if they are interested in a specific prompt, and finally to repeat this process till the group has achieved a certain degree of familiarity. 

In this paper, we introduce \sys{}, a prototype application built for Slack to provide social groups with an online icebreaker experience. Taking advantage of the fact that many offline social groups (such as coworkers or neighbours), also inhabit some accompanying online platform (such as Slack or Nextdoor), \sys{} contributes a computationally-orchestrated mechanism that preserves individual agency in icebreaker experiences. \sys{} supports relationship building through group conversations that take place in short-lived Slack channels. Like many traditional icebreaker experiences, \sys{} catalyzes conversations by providing the group with discussion prompts. However, \sys{} differs in that it configures the participants in a conversation to only include those who have apriori expressed interest in the prompt. Instead of restricting the group to predefined prompts, \sys{} also allows users to anonymously contribute their own prompts, to reflect what they want to talk about. \sys{} combines three interlinked components to support initial interactions, and more broadly, relationship building: (1) instead of being restricted to predefined prompts, it allows users to contribute topics they want to talk about to a queue of prompts that also includes predefined icebreaker prompts; (2) an engine that routinely gauges each user's interest in available conversation topics in the queue and launches conversations to include only those users who are interested in the topic; and (3) it provides users with awareness information about who they encounter most often in conversations orchestrated by \sys{}.   

To undestand, in-situ, how \sys{} and agency-preserving mechanisms can support relationship building among unacquainted individuals in social groups, we deployed \sys{} in a month-long pilot with a group of $N$ students beginning a summer undergraduate research program at a private research university. To do this, we collaborated with organizers of the program. As an instance of social groups of ``familiar strangers'', students in this group (1) \textit{how} they used \sys{}; and (2) the \textit{experience} of engaging in mutually involving conversations and the \textit{benefits} it provided



% To support social encounters between members of place-based communities, designers, artists, and researchers across various fields have investigated the design of installations, interventions, gadgets, and furniture 
% Social technologies such as NextDoor, Facebook Neighbourhoods, and Slack extend neighbourhoods and workplaces by providing them an online venue, while also creating opportunities to strengthen the local communities. However, in designing these social technologies, researchers have places an outsize importance on \textit{maintenance of relationships} by focusing on providing awareness that can support informal interactions, spontaneous knowledge sharing, and opportunistic encounters


-Icebreaker experiences contribute arbitrary shared focii
-Instead, we reveal common ground

-People are more self-conscious when interactions are forced. Because they have more control in when how 

-Nooks is a leveling mechanism that blurs other social boundaries

-Justify why online is good
-springboard for subsequent discussion
-Why is icebreaking the solution




==> sections-old/01_introduction_v1.tex <==
Researchers, designers, and artists have demonstrated the potential of icebreaker experiences to help people initiate interactions with others in their social groups, including those with whom they may be unacquainted ~\cite{karahalios2004telemurals, hespanhol2014using, chlup2010breaking, depping2016trust, sileo1998strategies, trotto2013engage}. Whether we are attempting to get to know other residents in our dormitory or other coworkers in our office, across a range of personal and professional contexts, we commonly find ourselves having to initiate interactions with people we have not previously met but with whom we hope to develop a relationship. Even when there is a mutual desire to interact and develop familiarity, initiating interactions with new connections can be challenging for many~\cite{mitchell2019facilitating}. The difficulty arises from the fact that ``interactions do not simply begin'': individuals must figure out \textit{what} to talk about, with unfamiliar others~\cite{haugh2021pragmatics}. Icebreaking experiences bring people together, and employ various conversational catalysts including installations, interventions, and physical artefacts that contribute \textit{what} a group can talk about.  

Unfortunately the same designed orchestration that is intended to support initial interactions, can also limit the effectiveness of icebreaking experiences: conversational prompts impede formation of closeness if participants are thrust into conversations they personally find uninteresting or inappropriate. Icebreaking experiences attempt to eliminate barriers around \textit{what} to talk about by providing predefined conversational prompts. However, because they do not explicitly account for what each participant is willing to talk about, icebreaking prompts can lead to situations where some participants in a conversation find the prompt uninteresting, irrelevant, or even inappropriate. Successful evolution of early relationships requires a contextually suitable level of sharing from individuals accompanied by reciprocal sharing from others in the conversations~\cite{miller2021meeting, sprecher2013taking}. However, if some participants find the prompt inappropriate or irrelevant, it can prevent them from reciprocating the self-disclosures they receive from others. Relatedly, when participants in a conversation fear that others might be uninterested and may not reciprocate their self-disclosures, they may choose not to participate altogether.

Icebreaking experiences could better support early relationship formation if they were designed to facilitate conversations in which it was ensured that participants shared a desire to participate, and if this shared desire was made explicit to all participants. When all participants in the conversation are interested in the topic, risk of non reciprocation is lower. Further, explicitly communicating the existence of shared interest can eliminate the fear of non reciprocation, while also fostering similarity-based affection. However, manually orchestrating such interest-based conversations between individuals can be cumbersome, requiring effort to source potential topics of interest, to find out who is interested in what topics, and finally to repeat this process multiple times because relationship building often requires multiple interactions. 

In this paper, we introduce \sys{}, a computationally-driven icebreaker mechanism that supports early relationship building in social groups of unacquainted people, by orchestrating interest-based conversations. Today most, if not all, offline groups use online messaging platforms to supplement their offline interactions and so, initial interactions can take place both online and offline. \sys{} is a prototype system built for one such common online messaging platform---Slack--- but  that extends Slack with a venue for    Because users know what they themselves are willing to interact about, \sys{} combines three interlinked components to support initial interactions, and more broadly, relationship building: (1) it allows users to contribute topics they want to talk about to a queue of prompts that also includes predefined icebreaker prompts; (2) an engine that routinely gauges each user's interest in available conversation topics in the queue and launches conversations to include only those users who are interested in the topic; and (3) it provides users with awareness information about who they encounter most often in conversations orchestrated by \sys{}  





% To support social encounters between members of place-based communities, designers, artists, and researchers across various fields have investigated the design of installations, interventions, gadgets, and furniture 
% Social technologies such as NextDoor, Facebook Neighbourhoods, and Slack extend neighbourhoods and workplaces by providing them an online venue, while also creating opportunities to strengthen the local communities. However, in designing these social technologies, researchers have places an outsize importance on \textit{maintenance of relationships} by focusing on providing awareness that can support informal interactions, spontaneous knowledge sharing, and opportunistic encounters



==> sections-old/01_introduction_v2.tex <==
Whether we are attempting to get acquainted with other residents in our dormitory or other coworkers in our office, in many social groups we are part of across personal and professional contexts, we commonly find ourselves wanting to initiate interactions and develop relationships with ``familiar strangers''~\cite{paulos2004familiar, milgram1977familiar}---described by social psychologist Stanley Milgrim as people we regularly observe but do not interact with. Social relationships within a group can have far-reaching consequences---they transform a group into a source of social support and enhance well-being by allowing those in the group to derive positive meaning from their participation in it. However, even when there is a mutual desire to interact and develop familiarity, initiating interactions with familiar strangers can be challenging for many~\cite{mitchell2019facilitating, olsson2020technologies, mitchell2019levelling, exley2004small, jarusriboonchai2016design}. The difficulty arises from the fact that ``interactions do not simply begin'': individuals must figure out what to talk about, with unknown others~\cite{haugh2021pragmatics, olsson2020technologies}. 

Researchers, designers, and artists have demonstrated the potential of designed icebreaker experiences to help relationship building in social groups,
% including those with whom they may be unacquainted
~\cite{karahalios2004telemurals, hespanhol2014using, chlup2010breaking, depping2016trust, sileo1998strategies, trotto2013engage}.
Designed icebreaker experiences use online and offline approaches to bring people together and spark conversations by providing the group with a conversation-starter~\cite{ludvigsen2005designing}. They provide this conversation-starter in various forms---discussion prompts~\cite{sileo1998strategies, chlup2010breaking}, installations~\cite{karahalios2004telemurals, snibbe2009social, hespanhol2014using}, gadgets~\cite{paulos2004familiar, mitchell2015sensing}, and even games~\cite{jarusriboonchai2016design, nasir2013cooperative}---and occasionally even sequence conversation-starters to spark increasingly intimate interactions. Through this designed scaffolding, they contribute \textit{what} a group can talk about and aim to support progressive development of familiarity, solidarity and closeness. [One sentence about how prompts can icrease likelihood of someone saying something] 

Unfortunately the same designed scaffolding that is intended to support initial interactions, can also limit the effectiveness of icebreaking experiences: conversation-starters and sequences impede formation of closeness if some participants are forced into conversations they don't \textit{want} to have. Icebreaking experiences attempt to eliminate barriers around what to talk about by enforcing predefined conversation-starters and sequences. However, even if participants are interested in the icebreaking experience as a whole, they may not be fully informed of the specific interactions that are to follow--- icebreaking experiences don't explicitly account for what each participant is willing to talk about, in a given group and at a certain point in time. As a result of this, icebreaking experiences can lead to situations where some participants in a conversation find the the topic uninteresting, irrelevant, or even inappropriate~\cite{miller2021meeting, rogers2002subtle}. Successful evolution of early relationships requires self-disclosures accompanied by reciprocal self-disclosures from others in the interaction~\cite{miller2021meeting, sprecher2013taking, svennevig2014direct}. However, if some participants find the conversation inappropriate or irrelevant, it can prevent them from sharing as well as reciprocating the self-disclosures they receive from others~\cite{miller2021meeting}. Additionally, when participants in an interaction fear that others might be uninterested and may not reciprocate their self-disclosures, they may choose not to participate themselves. Because they risk placing participants in conversations they find uncomfortable, designed icebreaker experiences---despite their benefits---can often fail at their goal of relationship building.

We propose that icebreaker experiences can better support early relationship formation in social groups if they guarantee that conversation-starters are \textit{mutually involving}: that everyone in the conversation shares a desire to interact on the topic. When all participants in an interaction want to participate, risk of non reciprocation is lower. By assuring participants in a conversation that everyone else also \textit{wants} to talk about the topic, a guarantee of mutual involvement, can alleviate fears of non-reciprocity and also foster similarity-based affection, both of which can support relationship building~\cite{svennevig2014direct}.

In this paper, we introduce a new system that supports relationship building in social groups by iteratively bringing individuals across a group in contact with each other over \textit{mutually involving} conversations. Taking advantage of the fact that many offline social groups (such as coworkers or neighbours), also inhabit some accompanying online platform (such as Slack or Nextdoor), we present \sys{}, a prototype application built for Slack that supports relationship building through group conversations that take place in short-lived Slack channels. To support relationship building in groups through \textit{mutually involving} conversations, \sys{} must simultaneously ensure that (1) each person has opportunities to participate in conversations they find interesting; and (2) each conversation is restricted to participants who are interested in participating in it. Because a static set of conversation-starters can't adequately capture the diverse and evolving interests of individuals in a group, to ensure participation opportunities, \sys{} provides people with controls to anonymously suggest their own conversation-starers. To configure participants in a conversation, \sys{} provides individuals with controls to decide for themselves which conversations they are interested in. Underlying \sys{} is a computationally-orchestrated mechanism that continually aggregates these preferences and launches conversations. \sys{} combines three interlinked components to support initial interactions, and more broadly, relationship building: (1) an engine that routinely gauges each user's interest in available conversation-starters and launches conversations to include only those users who are interested in the topic; (2) instead of being restricted to a static list of conversation-starters, it allows users to anonymously contribute topics they want to talk about; and (3) it provides users with awareness information about who they encounter most often in conversations orchestrated by \sys{}. \sys{} answers previous calls for icebreaker experiences that are not over-prescriptive and allow participants to appropriate and avoid interactions has been previously acknowledged~\cite{mitchell2019levelling, rogers2002subtle}.

To undestand, in-situ, how \sys{} and agency-preserving mechanisms can support relationship building among unacquainted individuals in social groups, we deployed \sys{} in a month-long pilot with a group of $N$ students beginning a summer undergraduate research program at a private research university. To do this, we collaborated with organizers of the program. As an instance of social groups of ``familiar strangers'', students in this group (1) \textit{how} they used \sys{}; and (2) the \textit{experience} of engaging in mutually involving conversations and the \textit{benefits} it provided

==> sections-old/01_introduction_v5.tex <==




At work, we commonly find ourselves wanting to develop relationships with ``familiar strangers''~\cite{paulos2004familiar, milgram1977familiar}---described by social psychologist Stanley Milgram as people we regularly observe but do not interact with. Strong social relationships within a group can have far-reaching consequences, transforming a group into a source of social support and enhance well-being by allowing individuals to derive positive meaning from their participation in the group. 

However, even when there is a mutual desire to interact and develop familiarity, initiating interactions with familiar strangers can be challenging for many~\cite{mitchell2019facilitating, olsson2020technologies, mitchell2019levelling, exley2004small, jarusriboonchai2016design}. Because they share little knowledge about each other, unacquainted individuals can struggle to identify what to talk about with each other~\cite{haugh2021pragmatics, olsson2020technologies}. Common ground between individuals---comprising common expertise and interests---that can form the basis of initial interactions is often invisible. Attempting to search for and confirm topics of common ground, involves risks. Individuals can risk appearing intrusive, rude, or impolite in attempts to infer common ground. These frictions can deter people from initiating interactions and as a result, developing relationships with others.

What if social evaluation of interests didn't incur embarrassment? This paper introduces a new system, Nooks, that supports relationship building in social groups by iteratively enabling individuals across the group, to discover and interact with others they share common ground with. \sys{} is a continually-running system that presents individuals with an evolving pool of conversation topics.  Members of the group can anonymously contribute topics to, and probes their interest in a group in topics that interest them. Nooks enables members to find other members in a group interested in a topic, and launch conversations with only include those individuals who have expressed interest in the topic, \sys{} unites individuals over the common ground they share---topics of shared interests. \sys{} attempts to lower the perceived risks of initiating interactions by guaranteeing individuals in a conversation that the conversation is mutually involving: that everyone in it wants to interact on the topic. 

\sys{} is a piggyback prototype built on Slack. Taking advantage of the fact that many offline social groups (such as coworkers or neighbours) already inhabit some accompanying online platform (such as Slack or Nextdoor), \sys{} contributes an instantiation of how existing infrastructure can be extended to reveal common ground and enhance opportunities for online and offline interactions in social groups. \sys{} brings individuals that share common interests in contact with each other over conversations in short-lived Slack channels. To discover common ground, \sys{} combines two interlinked components: (1) it allows users to contribute topics they want to talk about to a pool of conversation topics; and (2) an engine that routinely probes each user's interest in available conversation topics in the pool and launches conversations to include only those users who are interested in the topic.



% We suggest an alternative approach: instead of enforcing conversation-starters and sequences, allow participants to propose what they \textit{want to} talk about and provide them with the choice to opt in to \textit{specific} interactions they want to participate in. When all participants in an interaction want to participate, risk of non reciprocation is lower. Such a mechanism, intuitively, communicates to everyone in an interaction that the interaction is \textit{mutually involving}: that everyone in the conversation shares a desire to interact on the topic. This can alleviate fears of non-reciprocity and also foster similarity-based affection, both of which can support relationship building~\cite{svennevig2014direct}. The need for icebreaker experiences that are not over-prescriptive and allow participants to appropriate and avoid interactions has been previously acknowledged~\cite{mitchell2019levelling, rogers2002subtle}.

% However, manually orchestrating such a mechanism in a group can be cumbersome, requiring effort to source potential interaction prompts, periodically check with each person if they are interested in a specific prompt, and finally to repeat this process till the group has achieved a certain degree of familiarity. 

To undestand, in-situ, how \sys{}  can support relationship building among unacquainted individuals in social groups, we deployed \sys{} in a nine-week pilot with a group of $25$ students beginning a summer undergraduate research program. As an instance of social groups of ``familiar strangers'', students in this group (1) \textit{how} they used \sys{}; and (2) the \textit{experience} of engaging in mutually involving conversations and the \textit{benefits} it provided



% To support social encounters between members of place-based communities, designers, artists, and researchers across various fields have investigated the design of installations, interventions, gadgets, and furniture 
% Social technologies such as NextDoor, Facebook Neighbourhoods, and Slack extend neighbourhoods and workplaces by providing them an online venue, while also creating opportunities to strengthen the local communities. However, in designing these social technologies, researchers have places an outsize importance on \textit{maintenance of relationships} by focusing on providing awareness that can support informal interactions, spontaneous knowledge sharing, and opportunistic encounters


-Icebreaker experiences contribute arbitrary shared focii
-Instead, we reveal common ground

-People are more self-conscious when interactions are forced. Because they have more control in when how 

-Nooks is a leveling mechanism that blurs other social boundaries

-Justify why online is good
-springboard for subsequent discussion
-Why is icebreaking the solution


TODO: Need also in what ways Nooks was unsuccessful. 

TODO: Need an end sentence that says what Nooks tells you about the process of building systems to help social inclusion/relationship building more generally. 

==> sections/03_design_new.tex <==
%Sign posting: first we provide a system overview, and then we describe in more detail three (?) core attributes of the Nooks system.

\sys{} is a system that supports relationship-building in workplaces by focusing on decreasing the friction inherent in suggesting and participating in initial interactions\cite{boothby2018liking, mitchell2019facilitating, olsson2020technologies, mitchell2019levelling, exley2004small, jarusriboonchai2016design}. The underlying premise of the system is a \textit{nook}---a conversation room  with a defined focus hosting interested users while hiding the identity of the creator. We implemented the prototype of this approach as a Slack application because many organizations already use Slack or similar online messaging platforms\cite{10.1145/2818052.28691, 10.1145/3272973.3274060 }, and thus it may be smoothly integrated into various workplaces. The \sys{} Slack bot manages a dynamic daily pool of nooks to which anyone in the respective Slack workspaces can anonymously contribute to. To discover interested users, each nook goes through an incubation period during which individuals across the group are probed about their interest in joining it; users may opt-in or opt-out of conversations as they see fit. After this incubation period, the nook is launched as a temporary Slack channel adding everyone that has expressed interest, as channel members, all at once. By joining nooks that they are interested in, individuals thus explicitly signal their interest in the topic for the specific time-period when the channel is active to other participants and are brought in contact with others who have signalled a similar interest---including the creator--thereby establishing a mutual awareness of a shared interest---a common ground. Taken together, anonymous creation of nooks, ensuring an interested audience before a conversation starts, and making the process of actively finding common ground a norm in this alternate communication framework helps \sys{} lower the burden of initial interactions experienced by its users. 
Next, we describe a sample scenario of how \sys{} can be used to initiate interactions within a group. Then, we describe the features of the system, focusing on: (1) how users can make ongoing contributions to the pool of nooks through the \sys{} homepage (Figure \ref{fig:interface}); and (2) how the continually-running engine routinely probes individuals' interest and launches nooks, with the flow shown in Figure \ref{fig:flow}. Then, we discuss the implementation of \sys{} and conclude by describing how \sys{} can be adopted by workplaces in practice.

\subsection{Example scenario: initiating affinity groups at work}

Jos\'e has recently joined a new design agency. As someone that enjoys reading mystery novels, Jos\'e is interested in finding others at work with whom he can exchange recommendations and discuss books. He is connected to others through Slack and also has opportunities to approach them in person but he is unsure about who might be interested, and whether people would find his invitation appropriate. So, he decides to use \sys{} to discover others who are interested in mystery novels. To do this, Jos\'e simply creates an anonymous nook on mystery novels (\textit{sourcing and representing interests as nooks}), and in the description, clarifies his intentions to use the space to exchange recommendations and discuss books. Through the incubation period, \sys{}' execution engine accumulates others' interest in joining the conversation (\textit{convening individuals interested in a nook through routine aggregation of individual interests}). Finally, at the end of the incubation period, Jos\'e is added to a 24 hour conversation with others who have also expressed interest in the nook. Everyone in the conversation knows that they share an interest in mystery novels and so, they feel comfortable exchanging recommendations. They hop in and out of the conversations as they find time while the nook is alive. After their interaction, the group members have discovered a common love for mystery novels and this interaction acts as a starting point for some future connections.

%Jos\'e has recently joined a new design agency. Jos\'e is interested in finding others with common interests and building connections at work. He is connected to others through Slack and also has opportunities to approach them in person but he is unsure about who might be interested, and whether people would find his invitation appropriate. So, he decides to use \sys{} to discover others who are interested in mystery novels as a way to initiate interactions with others. To do this, Jos\'e simply creates an anonymous nook on mystery novels (\textit{sourcing and representing interests as nooks}), and in the description, clarifies his intentions to use the space to exchange recommendations and discuss books. Through the incubation period, \sys{}' execution engine accumulates others' interest in joining the conversation (\textit{convening individuals interested in a nook through routine aggregation of individual interests}). Finally, at the end of the incubation period, Jos\'e is added to a 24 hour conversation with others who have also expressed interest in the nook. Everyone in the conversation knows that they share an interest in mystery novels, that the nook is a specialized place for this purpose and so, they feel comfortable exchanging recommendations. They hop in and out of the conversations as they find time while the nook is alive. After their interaction, Jos\'e has discovered multiple co-workers with whom he shares a common ground and this interaction acts as a starting point for some future connections. 

\subsection{Sourcing and representing topics of conversation as nooks}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/Interface.pdf}
    \caption{The study workflow and data collected in the different stages of the study.}
    \label{fig:interface}
\end{figure}
For \sys{} to bring people in contact with each other over common interests, it needs a representation of people's interests that it can then use to connect individuals. What people want to talk about with others is often context specific and evolving, varying with the nature of interpersonal relationships as well as surrounding context. To capture individuals' evolving interests in a way that can be used to attract like-minded others, \sys{} lets users anonymously create nooks whenever they want, by providing a topic for the nook and a description of what they want to talk about within it. [why is this better than other topic sourcing] [why is anonymity good] 
% short lived nature 
% By default all nooks are archived after 24 hours to encourage this evolving and more specific nature of such topics of interest while ensuring critical mass. However, members can unarchive the channels if they want this interaction to be more long lived.  
To create a new nook, users can proceed to the ``Create a Nook" panel in the Nooks home page (Figure \ref{fig:interface}) within Slack. Clicking on ``Create a Nook" (A1) opens an overlay form (A4) asking the user to describe nook they want to create. Specifically, they are asked to provide a `title' and their `initial thoughts'. Here they can describe not just \textit{what} they want to talk about but also what they want the norms of the conversation to be. By default, nooks are open for anyone in the group to join, however, the creator can optionally select specific users they don't want included. Many early users of \sys{} voiced a need for such a control to minimize the scope of unwanted interactions. When only one other person that expresses interest in the \sys{}, launching of the nook implicitly reveals the creator. While creators are not identified during the incubation of a nook, if the creator wants to additionally remain anonymous even after the nook has been launched, they can opt to have the nook created only if there are atleast two other individuals in it. Finally, they can create the nook by clicking the 'Add Nook to the Queue' button at the bottom of the overlay(A5). This panel also shows users a variety to pre-populated sample nooks to inspire users. They can navigate through these samples by clicking on ``Get more samples" (A2). Clicking the "Edit and Use" button (A3) opens the overlay form (A4) with the corresponding sample as an editable Nook title. 

% \subsubsection{Community organizers facilitating icebreaking}
% To increase their opportunities for connection, the program coordinators have also invited the students to a Slack workspace where they can interact even when physically distant.
% To enhance opportunities for students to get to know each other, the program coordinators decide to use an icebreaker tool, \sys{}, to provide students with an icebreaker experience. After introducing the application to the students and adding it to their Slack workspace, for a few weeks the program coordinators feed the application with a daily discussion prompt that they would like to \textit{suggest}, but not \textit{enforce}. \sys{}' execution engine asks each student if they would like to join a conversation around the prompt scheduled for the next day. Jose is interested in joining the conversation for one such prompt---``share an embarrassing
% moment in your life''. He thinks it will be a playful way to get to know others better. Maya, on the other hand, does not yet feel comfortable enough with other students to participate in the conversation and opts out of the conversation\footnote{Previous work has found that people rating higher on an introversion scale tend to shy away from more intimate conversations~\cite{nguyen2015known}.}. Jose is added to the conversation the next day, and he enjoys an engaging conversation with other interested students. Because there is ambiguity about whether Maya opted out or whether she simply missed the notification, her absence in the conversation does not bother those in it. 

% \subsubsection{\sys{} as a way to initiate affinity groups}

% % Next, we outline a motivating scenario to demonstrate our goals for a system that reveals common ground. Jose and Maya are among a new cohort of students joining a graduate program in a design department. Students in the cohort are demographically diverse and come from different backgrounds and different cities, most having relocated to start in the program. New to the department, the city, and each other, most students in the cohort are hoping to get to know each other. The department's building serves as a backdrop for a number of encounters between students: they see others attending the same classes or department events, and they routinely encounter each other when working in the common spaces. Encounters are usually opportunistic as students have the flexibility to work wherever and whenever they prefer.  However, across the offline encounters and broadcast communication on Slack, Jose and Maya have been unable to get to know their cohort as well as they would have liked to. Like many others in their cohort, Jose and Maya feel disconnected from students in their cohort.   



% When the execution engine presents Maya with the potential conversations she can participate in the next day, she notices a prompt on exchanging design feedback. She is excited about getting feedback on her designs while also helping others, and becoming familiar with them in the process. She expresses interest in joining the conversation and the next day she is added to the conversation where she is introduced to Jose. After few weeks of using \sys{}, Jose notices that Maya and he have interacted several times within \sys{}. The next time he needs someone to give him feedback on his designs, he reaches out to Maya directly. 

\subsection{Convening individuals interested in a nook through routine aggregation of individual interests}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/flow.pdf}
    \caption{The flow of a nook through the executions engine}
    \label{fig:flow}
\end{figure}

Using a user-contributed nook to then assemble a group of people interested in it, requires a mechanism that probes people across the workspace about their interest in joining it. Within \sys{}, each user-contributed nook is ``incubated''---other users across the group are shown the topic and description of the nook and asked for their interest in joining a nook. Next, we describe how nooks are incubated and launched.
\subsubsection{Incubation and launch}
When a nook is being incubated, it is displayed on the \sys{} homepage (panel B in Figure \ref{fig:interface}) for all members across the workspace, excluding those who the creator has requested to exclude. Users can click `interested' or `not for me'(B2) on each nook they are shown (B1). If multiple nooks are being incubated at the same time, they are shown one after the other. \sys{} records each user's choice. At the end of the incubation period, each nook is launched as a Slack channel to which the \sys{} bot automatically adds all users who had expressed interest, and posts the topic and the description as the first message in the created channel. 

Slack channels that host nooks are always launched at 12pm and are open for 24 hours, after which they are automatically archived. In keeping with best practices on the design of online spaces, this is done to establish a schedule of `expected active times', during which participants can expect each other to be active in the space~\cite{10.7551/mitpress/8472.003.0007} and consequently, promotes activity in a self-fulfilling way. Since users may not always be active on Slack, and diffused participation can impede conversations, we establish expected times of activity in attempts to promote engaging conversations. Participants are notified when the conversation is archived and if participants in a conversation want to convert the nook into a more persistent space, they have the option to unarchive the channel. We chose to launch nooks at 12pm because that was the time by which most people in our pilots had started their work day, however, this time could be customized to a workplace depending on the distribution of times when individuals start their work day.

\subsubsection{Incubation and notification routine}
\sys{} houses communities at the scale of a workplace and so, interaction opportunities---incubating nooks---within it can be sparser than interaction opportunities---such as discussion threads---in large online communities. Prior work suggests that when interaction opportunities are sparser, users lower the frequency of their visits~\cite{10.7551/mitpress/8472.003.0007}, which can result in some incubating nooks going unnoticed. To ensure that incubating nooks are viewed by a sufficient number of users, we chose to use a \textit{push model} where users are notified when new interaction opportunities---incubating nooks---are available~\cite{10.7551/mitpress/8472.003.0007}. However, notifying individuals every time a nook is created can lead to excessive notifications. To simultaneously ensure that each nooks is viewed by a sufficient number of people and that the interruption cost of notifications is low, we devised a temporal routine according to which nooks are incubated in batches. Figure \ref{fig:flow} shows this routine. All nooks created before 4pm on any given day are added to that day's incubation batch and are incubated together from 4pm that day to 12pm the following day. Users are notified that a new batch of incubating nooks is available via a Slack message triggered by the application (Figure \ref{fig:interface}). Nooks being incubated together are displayed sequentially to users on the homepage. At 12pm the following day, incubating nooks are launched as Slack channels including all members who have expressed interest in it by then. Nooks created after 4pm are added to the following day's incubation batch. 

\subsection{Implementation}
Nooks is a Slack application and a companion Slack bot, implemented in Python with a Flask  back-end. We used the Slack Bolt API to create the Slack interface and monitor events triggered as users interact with the bot. The back-end was served on a Digital Ocean instance with a MongoDB database. To maintain participants' privacy, we did not log any conversations. We only collected participant's demographic data when they created their profile, and for every nook created, we recorded the title and details of the nook created, the user ID of the creator, the user IDs of those who expressed interest and disinterest in the nook, and finally user IDs are all members who were added to the nook. Participants had to sign a consent form before signing up explaining the process and the data collected. The project is open source and available at https://anonymous.4open.science/r/Nooks-18CC [anonymized for submission]. 


\subsection{Adopting, customizing, and promoting use within a workplace}
% We assume a workplace has been instituted
We envision \sys{} as a tool that workplace administrators and decision-makers---those responsible for making workplace-wide decisions---can adopt for their workplace as a way to support relationship building in the workplace. Like most social computing systems, for \sys{} to be useful as a tool for initial interactions, individuals across the workplace need to sign-up as and actively use the application. Once installed in the Slack workspace of the workplace, \sys{} allows administrators to onboard members from a specific channel in the workplace, to control who participates in \sys{}. Onboarding members from the general channel, for instance, would onboard everyone in the Slack workspace. Alternately, they can also invite specific members based on their Slack usernames. \sys{} sends invited users a Slack message, walking them through the sign-up process. 

Finally, to promote the use of the application, administrators can create a predefined set of nooks that are inserted into the application during set-up. Allowing users to view and join these predefined nooks, provides them with interaction opportunities even before they have created their own nooks. When populated with predefined nooks, by administrators, \sys{} acts similar to systems that deliver online icebreaking prompts to groups. However, they differ in that prompts are only \textit{suggested}, not \textit{enforced}: users make decisions about what conversations they join. Participating in predefined nooks also supports users in learning \sys{}' underlying mechanism and allows them to experience conversations in a nook which can inform their decision to create their own. 


% customize the application to the context of their workplace. 

% Below, we describe: (1) tools for onboarding users on \sys{}; (2) aspects of nooks that can be customized to the workplace; and (3) strategies to promote use informed by our experience.

% -requires institutioning 
% -can customize the edit+use
% -can 



==> sections/motivating-scenarios.tex <==
Next, we outline a motivating scenario to demonstrate our goals for a system that reveals common ground. Jose and Maya are among a new cohort of students joining a graduate program in a design department. Students in the cohort are demographically diverse and come from different backgrounds and different cities, most having relocated to start in the program. New to the department, the city, and each other, most students in the cohort are hoping to get to know each other. The department's building serves as a backdrop for a number of encounters between students: they see others attending the same classes or department events, and they routinely encounter each other when working in the common spaces. Encounters are usually opportunistic as students have the flexibility to work wherever and whenever they prefer. To increase their opportunities for connection, the program coordinators have also invited the students to a Slack workspace where they can interact even when physically distant. However, across the offline encounters and broadcast communication on Slack, Jose and Maya have been unable to get to know their cohort as well as they would have liked to. Like many others in their cohort, Jose and Maya feel disconnected from students in their cohort.   

To enhance opportunities for students to get to know each other, the program coordinators decide to use an icebreaker tool, \sys{}, to provide students with an icebreaker experience. After introducing the application to the students and adding it to their Slack workspace, for a few weeks the program coordinators feed the application with a daily discussion prompt that they would like to \textit{suggest}, but not \textit{enforce}. \sys{}' execution engine asks each student if they would like to join a conversation around the prompt scheduled for the next day. Jose is interested in joining the conversation for one such prompt---``share an embarrassing
moment in your life''. He thinks it will be a playful way to get to know others better. Maya, on the other hand, does not yet feel comfortable enough with other students to participate in the conversation and opts out of the conversation\footnote{Previous work has found that people rating higher on an introversion scale tend to shy away from more intimate conversations~\cite{nguyen2015known}.}. Jose is added to the conversation the next day, and he enjoys an engaging conversation with other interested students. Because there is ambiguity about whether Maya opted out or whether she simply missed the notification, her absence in the conversation does not bother those in it. 

As someone that enjoys horror films, Jose decides to use \sys{} to initiate an interaction with other students interested in horror films, both as a way to interact with others about a shared interest and to initiate a plan to watch a film with others. To do this, Jose simply feeds \sys{} with an anonymous prompt on horror films. The execution engine, by gauging others' interest, assembles a group of students interested in talking about horror films and creates a conversation with Jose included. \sys{} doesn't identify the creator of the conversation and so, it doesn't burden Jose with the responsibility of facilitating the interaction. Everyone in the conversation knows that they share an interest in horror films and so, they exchange recommendations and few of them plan a movie night.

When the execution engine presents Maya with the potential conversations she can participate in the next day, she notices a prompt on exchanging design feedback. She is excited about getting feedback on her designs while also helping others, and becoming familiar with them in the process. She expresses interest in joining the conversation and the next day she is added to the conversation where she is introduced to Jose. After few weeks of using \sys{}, Jose notices that Maya and he have interacted several times within \sys{}. The next time he needs someone to give him feedback on his designs, he reaches out to Maya directly. 
